MADE: Graph Backdoor Defense with Masked Unlearning

Graph Neural Networks (GNNs) have garnered significant attention from researchers due to their outstanding performance in handling graph-related tasks, such as social network analysis, protein design, and so on. Despite their widespread application, recent research has demonstrated that GNNs are vulnerable to backdoor attacks, implemented by injecting triggers into the training datasets. Trained on the poisoned data, GNNs will predict target labels when attaching trigger patterns to inputs. This vulnerability poses significant security risks for applications of GNNs in sensitive domains, such as drug discovery. While there has been extensive research into backdoor defenses for images, strategies to safeguard GNNs against such attacks remain underdeveloped. Furthermore, we point out that conventional backdoor defense methods designed for images cannot work well when directly implemented on graph data. In this paper, we first analyze the key difference between image backdoor and graph backdoor attacks. Then we tackle the graph defense problem by presenting a novel approach called MADE, which devises an adversarial mask generation mechanism that selectively preserves clean sub-graphs and further leverages masks on edge weights to eliminate the influence of triggers effectively. Extensive experiments across various graph classification tasks demonstrate the effectiveness of MADE in significantly reducing the attack success rate (ASR) while maintaining a high classification accuracy.

==> 03method2.tex <==
\section{Methodology}
In this section, we first point out some potential drawbacks of some traditional backdoor defense methods for images when used for graphs. Furthermore, based on this understanding, we propose an effective method, \method, to defend against backdoor attacks on graphs.

\subsection{Drawbacks of Backdoor Defenses for Images}
Typical backdoor defense methods always explore how to defend against attacks with deep neural networks (DNNs) under image datasets. However, the parameters of networks and the scale of datasets vary greatly between images and graphs. Specifically, the layers of GNNs are much smaller than those of DNNs, and the datasets of graphs are smaller than those of images. Therefore, it is hard for typical backdoor defense methods to perform well when faced with state-of-the-art graph backdoor attack methods.

To be specific, existing erasing works on image backdoor defenses can be categorized into three groups: (1) \textit{fine-tuning} attempt to eliminate the poisoned part of models by adjusting the parameters of models with clean datasets; (2) \textit{pruning} aims to identify and remove the contaminated neurons in models to cleanse the injected backdoor, and (3) \textit{unlearning} aim to adversarially reduce the model's performance on poisoned samples to effectively remove the backdoor.
 
However, all the methods mentioned above have their drawbacks. \textit{Fine-tuning} only has limited effects on defending and fails to perform well when faced with SOTA backdoor attack methods especially when the number of clean samples for fine-tuning is not enough. \textit{Pruning} performs badly on small networks. A typical example is Adversarial Neural Pruning (ANP) \citep{wu2021adversarial}, which utilizes adversarial perturbations to detect and prune suspicious poisoned neurons. Unfortunately, the effectiveness of ANP significantly deteriorates when applied to models with a small number of parameters. It is because in models with fewer parameters, a single neuron may be responsible for extracting multiple features, perhaps both the malicious and clean features. Consequently, pruning the neurons solely responsible for extracting the malicious features becomes extremely challenging, or even impossible. In traditional deep neural networks (DNNs), which often consist of tens of layers and have relatively large model sizes, ANP can effectively defend against backdoor attacks. However, graph neural networks (GNNs) typically have only 2 to 3 layers with a small number of parameters. As a result, \textit{pruning} struggles to achieve significant efficacy in GNNs.

Additionally, \textit{unlearning} also fails to have a satisfactory performance due to the disparity in learning difficulties between graph triggers and image triggers. The most commonly used method of \textit{unlearning} is Anti-backdoor Learning (ABL)\citep{li2021anti}. ABL initially selects a subset of contaminated data by exploiting the discrepancy in convergence rates of loss function between poisoned and clean samples. However, because of complex topology structures of graphs, poisoned graph data have a much lower convergence rate of loss function, which makes ABL hard to select poisoned data. We will further discuss this issue in Section \ref{\method} in more detail. Moreover, ABL employs adversarial gradient updates on the selected contaminated data to facilitate unlearning. However, the scale of graph datasets are much smaller, and the selected dataset constitutes only a small fraction (e.g., $1\%$) of the entire dataset. Therefore, ABL only unlearn extremely limited samples, which may not effectively erase the malicious features but may instead interfere with the extraction of clean features.

In summary, traditional backdoor defense methods are not applicable to graphs. Moreover, the critical topological information has not been leveraged by those backdoor defense methods. Therefore, naturally, our objective is to explore and develop a method that effectively defends against backdoor attacks on graphs by utilizing topological information.

\subsection{\method} \label{\method}
In this section, we will first discuss how to enrich poisoned data, followed by an explanation of how to generate a defensive mask based on those enriched poisoned data.

\subsubsection{Data Enrichment}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/diff_converge_rate.pdf}
    \caption{Differences in the response of models attacked by image backdoor and graph backdoor attacks.}
    \label{fig:diff_converge_rate}
\end{figure}


First, we evaluate the data selection part in ABL when applying it to graph neural networks and find that their performance is not consistent on some kinds of neural networks as shown in Table~\ref{tbl:enrich_rate}. From the above results, we find it cannot successfully select suspicious poisoned data and create an enriched poisoned dataset. Therefore, the performance of ABL is not satisfying on some graph backdoor datasets. Therefore, we need to explore new features for data isolation to find backdoor graphs to remove.

Inspired by the former works~\cite{adv-relate-homo}, we explore the homophily behaviors of backdoor graphs and poison graphs. The homophily property for different graphs is shown in Table~\ref{tab:homo}. 
\begin{table}[tbp] 
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{c| cccc}
        \toprule
        % & \multicolumn{4}{c}{\textbf{w. Node Features}} & {\textbf{w/o. Node Features}}\\
         & \textbf{AIDS} & \textbf{PROTEINS} & \textbf{PROTEINS\_full} & \textbf{ENZYMES} \\%& \textbf{NCI1}
        \midrule
          \textbf{Backdoor} & $0.85\pm0.06$ & $0.9\pm0.05$ & $0.81\pm0.08$ & $0.83\pm0.05$ \\%& $0.71\pm0.06$\\
          \textbf{Clean} & $0.98\pm0.02$ & $0.99\pm0.01$ & $0.99\pm0.01$  & $0.99\pm0.02$ \\% & $0.86\pm0.05$\\
          % \textbf{MaskDefense} & 76.94\% & 86.72\% & 34.59\% & 77.42\% \\
        \bottomrule
    \end{tabular}
    % }
    \caption{The average(standard variation) homophily of backdoor graphs and clean graphs.}
    \label{tbl:enrich_rate}
\end{table}
From the table, one can see that the graph's homophily behavior for backdoor graphs and cleans are different. Therefore, we can use such a metric to split graph samples by splitting graphs whose homophily is not in the following region as backdoor graphs:
\begin{equation}
\begin{aligned}
(homo^{avg}_{\mathcal{G}} - homo^{std}_{\mathcal{G}}, homo^{avg}_{\mathcal{G}}+homo^{std}_{\mathcal{G}}),
\end{aligned}
\end{equation}
where $homo^{avg}_{\mathcal{G}}=\mathop{Average}(\{homo(g_i)| g_i \in\mathcal{G}\})$ and $homo^{std}_{\mathcal{G}}=\mathop{StD}(\{homo(g_i)| g_i \in\mathcal{G}\})$. However, selecting only with homophily metric is not enough. Therefore, we also use following loss function besides the homophily metric for selection:
\begin{equation}
    loss = CE\left(\mathbf{x}, y\right) \cdot sign \left(CE\left(\mathbf{x}, y\right) - \gamma \right),
\end{equation}
where $\gamma$ is a hyperparameter, $CE(\cdot)$ denote the cross entropy loss function, and $\mathbf{x}$ and $y$ denote samples and corresponding labels, respectively. In the warm-up phase, the loss of clean samples will fluctuate around the hyperparameter $\gamma$, while the loss of poisoned samples will decrease rapidly. Therefore, ABL is capable of distinguishing the poisoned samples when facing image backdoor attacks.

Nevertheless, in graph backdoor attacks, the response of models to trigger patterns is more complex and nuanced. Graph triggers are typically embedded in the topological structure of the graph, affecting the connections and relationships between nodes. As a result, the model's response to graph triggers involves not only local changes but also systemic alterations in the graph, making it more challenging to detect and mitigate the impact of the triggers.
% in graph datasets, the unique topology of each graph introduces variations in trigger patterns.
Therefore, graph neural networks with backdoors demonstrate more intricate response mechanisms to graph triggers compared to their counterparts in the image domain. 
% Consequently, the convergence speed of the poisoned samples noticeably diminishes, posing challenges for the successful application of ABL.
We demonstrate the difference in Figure \ref{fig:diff_converge_rate}. Figure \ref{fig:diff_converge_rate} (a), \ie, the left and middle panel, illustrates the heatmap visualization of backdoor attacks in the image domain. Obviously, models tend to exhibit more straightforward and localized attention to the trigger patterns embedded in the images, the bottom right corner, which implies that the gradients within the trigger region are notably higher in magnitude compared to the surrounding clean pixel regions. Firgure \ref{fig:diff_converge_rate} (b), the right panel, illustrates the distribution of gradient magnitudes for both malicious (backdoor) and clean nodes across all graphs with backdoor. The y-axis represents the magnitude values of the gradients, while the x-axis distinguishes between malicious and clean nodes. Obviously, a higher proportion of nodes with larger gradient magnitudes in the malicious nodes compared to the clean nodes. However, the overall distribution proportions of the two types of nodes appear to be relatively similar, without any significant visual differentiation which has been found in Figure \ref{fig:diff_converge_rate} (a). 
Therefore, it demonstrates that GNNs pay less attention on graph triggers, and exhibit complex mechanisms for graph backdoors. Consequently, the convergence speed of the poisoned samples noticeably diminishes, posing challenges for the successful application of ABL.

\begin{table}[h] 
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{c| ccccc}
        \toprule
         & \textbf{AIDS} & \textbf{PROTEINS} & \textbf{PROTEINS\_full} & \textbf{ENZYMES} & \textbf{NCI1}\\
        \midrule
          \textbf{ABL} & 34.00\% & 89.97\% & 10.11\% & 97.92\% & -\%\\
          \textbf{MaskDefense} & 98.11\% & 95.21\% & 91.78\% & 96.77\% & 83.51\%\\
          % \textbf{MaskDefense} & 76.94\% & 86.72\% & 34.59\% & 77.42\% \\
        \bottomrule
    \end{tabular}
    % }
    \caption{proportion of poisoned sample among enriched datasets. The higher the proportion, the more effective the enrichment method is.}
    \label{tbl:enrich_rate}
\end{table}


Considering the above drawback, we abandon the utilization of the sign function in ABL to keep the high loss for clean samples. Instead, we directly optimize the original cross-entropy loss function. Following an initial warm-up training phase, we compute the per-sample loss function and select the top $\alpha_1$ samples with the lowest loss as the enriched harmful sample set, denoted as $\mathcal{D}_{bad}$. Moreover, we select $\alpha_2$ samples with the highest loss as the enriched clean sample set, denoted as $\mathcal{D}_{clean}$. To assess the efficacy of our proposed enrichment, we conduct experiments using the GTA backdoor attack with an injection rate of $10.0\%$ on four distinct datasets. we evaluate the proportion of truly injected trigger samples in the enriched poisoned dataset. The experimental results, as shown in Table \ref{tbl:enrich_rate}, reveal that our proposed method consistently achieves a relatively high proportion of truly injected trigger samples, effectively identifying the poisoned samples. 

\subsubsection{Forward Propagation with Masks}
Since the structure of a graph is easy to learn and unlearn, directly unlearning whole graphs with triggers will also make GNN forget some important information and lead to worse performance as shown in Figure~\ref{fig:unlearn_mask}. From the figure, one can see that directly unlearning the whole graph will significantly harm GNN's performance. However, only unlearning the connection between trigger subgraphs and target labels can also purify the poisoned model with better natural accuracy remaining.

\begin{figure}[h]
    \centering
    \begin{minipage}[c]{0.455\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/Unlearn_wo_mask_PROTEINS.png}
    \subcaption{(a) Without Mask.}
    \end{minipage}
    \begin{minipage}[c]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/Unlearn_w_mask_PROTEINS.png}
    \subcaption{(b) With Mask.}
    \end{minipage}
    \caption{Unlearning Performance with and without Masks on PROTEINS. Mask here is the ground truth indicting whether the node is the trigger or not.}
    \label{fig:unlearn_mask}
\end{figure}

Therefore, we are going to introduce how to effectively defend against backdoor attacks using masking techniques. Actually, by altering the graph's topological structure, the mask can be utilized to defend against backdoor attacks while maintaining competitive utility in two aspects. First, theoretically, setting the weights of connections between malicious and benign nodes, as well as self-loop edges, to zero would render the malicious node features incapable of influencing the final global graph representations, thus effectively eliminating the trigger's impact. Second, those masked edges serve to selectively mask specific node features within the malicious graph while preserving the features of the benign nodes and their relevant topological structure. This implies that valuable information within the malicious graph can still be utilized for training purposes, thereby retaining a competitive prediction accuracy.

Inspired by the former works on the difference between the poison samples and natural samples~\cite{wu2022debiasing,tran2018spectral}, we first draw the spectrum for the features of natural nodes and poisoned nodes shown in Figure~\ref{fig:spectrum_nodes}.
\begin{figure}[h]
    \centering
    \begin{minipage}[c]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/PROTEINS.png}
    \subcaption{(a) PROTEINS.}
    \end{minipage}
    \begin{minipage}[c]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/PROTEINS_full_Spec.png}
    \subcaption{(b) PROTEINS full.}
    \end{minipage}
    \begin{minipage}[c]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/ENZYMES_full_Spec.png}
    \subcaption{(c) ENZYMES.}
    \end{minipage}
    \caption{The spectrum for clean nodes and backdoored nodes on different datasets.}
    \label{fig:spectrum_nodes}
\end{figure}

From the figures, one can see that the graph's backdoored nodes concentrate more on their top dimensions while the features for clean nodes distribute more uniformly in the data space. If we can learn a weighted project to project the node features away from the top singular space, we can easily classify backdoor nodes and natural nodes and then get the trigger subgraph. Thereby, we introduce a learnable projection head that projects node features onto these introduced malicious dimensions:

% Therefore, we propose a weight calculation approach based on node similarity. Prior research \cite{wu2022debiasing} has demonstrated that backdoor attacks fundamentally involve dimensionality expansion of features and perturbations along the newly added malicious dimensions. To address this, we introduce a learnable projection head that projects node features onto these introduced malicious dimensions:

\begin{equation}
    \mathbf{p}_i^{(k)} = \textbf{HEAD} \left( \mathbf{h}_i^{(k)} \right),
\end{equation}
where $\textbf{HEAD}$ denotes the learnable projection head. Please note that the mapping of clean node features to the malicious dimensions is expected to be a zero vector, \ie, $p_(v_clean)^((k))=0$. As a result, the inner product between the mapped clean node features and any other features should be zero vectors. Hence, through a 0-1 flip, we can leverage the similarity between nodes to judge whether a node is clean:

\begin{equation}
    score^{(k)}(v_i) = \textbf{AVERAGE} \left( 1 - sim(\mathbf{h}_i^{(k)}, \mathbf{h}_j^{(k)}) : v_j \in \mathcal{N}(v_i) \right),
\end{equation}
where $\textbf{AVERAGE}$ denote a average function and $sim(\mathbf{h}_i^{(k)}, \mathbf{h}_j^{(k)})$ represents the cosine similarity between the node features $\mathbf{h}_i^{(k)}$ and $\mathbf{h}_j^{(k)}$. Intuitively, a lower clean score indicates a higher probability of being regarded as malicious. Moreover, we nullify the edge weights for the top $\beta$ nodes that are more likely to be malicious, in order to eliminate their influence on models. For the remaining nodes, we employ the clean score of the edges as the mask:

\begin{equation} \label{eq:mask_express}
    \mathbf{m}^{(k)}_{i, j} = \left\{
    \begin{aligned}
        & 0,\qquad v_i \in \mathcal{V}_{bad} \  or \  v_j \in \mathcal{V}_{bad}\\
        & 1-sim(\mathbf{h}_i^{(k)}, \mathbf{h}_j^{(k)}), \qquad else
    \end{aligned}
    \right.
\end{equation}
where $\mathbf{m}_{i,j}^{(k)}$ represents the mask on the edge between the node $v_i$ and $v_j$ after $k$ message passing. After obtaining the mask, we treat the graph as a weighted graph for message passing (if the graph was already a weighted graph, we multiply the mask as a factor with the original edge weights). Mathematically, the message passing is modified as follows:

\begin{subequations}
    \begin{align}
        &\mathbf{a}_i^{(k)} = \textbf{AGGREGATION} \left(\{\mathbf{m}_{i, j}^{(k)} \cdot \mathbf{h}_j^{(k)}: v_j \in \mathcal{N}(v_i)\} \right). \\
        &\mathbf{h}_i^{(k+1)} = \textbf{COMBINE} \left(\{\mathbf{m}_{i, i}^{(k)} \cdot \mathbf{h}_i^{(k)}, \mathbf{a}_i^{(k)}\} \right).
    \end{align}
\end{subequations}

\subsubsection{Gradient Update}
Once we have obtained the mask for each graph, we proceed to update the gradients based on whether the graph belong to the enriched poisoned dataset $\mathcal{D}_{bad}$ or not. In the case where the graph belongs to enriched clean dataset $\mathcal{D}_{clean}$, we utilize the normal loss function $loss_{clean}$, such as the cross-entropy loss, to update the model and facilitate the learning of clean sample features:
\begin{equation}
    loss = loss_{clean} \left( \textbf{GNN} \left( \mathbf{X}, \mathbf{A}\right), y \right),
\end{equation}
where $\textbf{GNN}$ represents the GNN model to be trained.

For graphs belonging to the enriched poisoned dataset $\mathcal{D}_{bad}$, we employ an adversarial loss function, denoted as $loss_{adv}$, to deteriorate the model's performance on the malicious samples, effectively unlearning triggers. Mathematically, this process can be represented as follows:
\begin{equation}
    loss = loss_{adv} \left( \textbf{GNN} \left( \mathbf{X}, \mathbf{A}\right), y \right),
\end{equation}
where $loss_{adv} = -loss_{clean}$. All the above training process is guided by Algorithm \ref{algo:compre_process}. In a nutshell, we initially differentiate the samples based on the disparity in convergence rate between clean and malicious samples. Subsequently, for every graph we calculate edge masks which selectively eliminate malicious part of graphs and then determine whether to learn or unlearn the graph features.

% \begin{minipage}
\begin{algorithm}[htbp] \label{algo:compre_process}
    \SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \Input{a graph dataset $\mathcal{D}$, a $K$-layer GNN with parameter $\Theta$, a task-specific loss function $loss_{clean}$, an adversarial loss function $loss_{adv}$, the epochs of warm-up phase $epoch_{warm}$, the epochs of training phase $epoch_{train}$.}
    \Output{a backdoor-insensitive GNN with parameter $\Theta_{opt}$.}
    Initialize gradient-base optimizer $optim$\;
    \tcp{warm-up phase to split datasets.}
    \For{epoch = $1 \rightarrow epoch_{warm}$}{
        \For{every graph $\mathcal{G} = \{\mathbf{A}, \mathbf{X}, y\}$ in $\mathcal{D}$}{
        $l = loss_{clean} \left(\textbf{GNN}\left( \mathbf{A}, \mathbf{X}\right), y\right)$\;
        }
        update $\Theta$ by $optim$\;
    }
    Get the top $\alpha_1$ samples $\mathcal{D}_{bad}$ with the lowest loss $l$\;
    Get the top $\alpha_2$ samples $\mathcal{D}_{clean}$ with the highest loss $l$\;
    \tcp{train GNN with masks}
    \For{every graph $\mathcal{G} = \{\mathbf{A}, \mathbf{X}, y\}$ in $\mathcal{D}_{clean} \cup \mathcal{D}_{bad}$}{
        Get masks $m$ based on Eq. \eqref{eq:mask_express}\;
        \If{$\mathcal{G} \in \mathcal{D}_{bad}$}{
            $l =loss_{bad} \left(\textbf{GNN}\left( \mathbf{A}, \mathbf{X}\right), y \right) $\;
        }
        \Else{
            $l = loss_{clean} \left(\textbf{GNN}\left( \mathbf{A}, \mathbf{X}\right), y\right)$\;
        }
        update $\Theta$ by $optim$\;
    }
    $\Theta_{opt} = \Theta$
    \caption{\method Algorithm.}
\end{algorithm}

==> data.tex <==
\begin{table*}[h]
    \centering
    \caption{Precision and recall of isolated backdoor samples with changing isolation rates on AIDS. The higher the precision and recall, the more effective the data isolation is. \ming{May be curves are better?}\xiao{solved}}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc}
        \toprule
         \multirow{2}{*}{isolation rate } & \multicolumn{4}{c}{Recall ($\uparrow$)} & \multicolumn{4}{c}{Precision ($\uparrow$)}  \\
        \cline{2-9}
         & 5\% & 10\% & 15\% & 20\% & 5\% & 10\% & 15\% & 20\% \\
        \midrule
         ABL & 36.25 & 34.00	& 18.36	& 33.44 & 18.12	& 34.00 & 29.38 & 67.87 \\
         \method{} & \textbf{90.00}	& \textbf{82.00}	& \textbf{59.33}	& \textbf{47.50} & \textbf{45.00} & \textbf{82.00} & \textbf{89.00} & \textbf{95.00} \\
         Maximum & 100.00& 100.00& 66.67	& 50.00 & 50.00 & 100.00 & 100.00 & 100.00 \\
        \bottomrule
    \end{tabular}
    % }
    \label{tab:prec&rec_diff_rate}
\end{table*}


\begin{table}[tbp]
    \centering
    \caption{Graph classification results on datasets purified with data isolation. Higher is better ($\uparrow$) for ACC (white). Lower is better ($\downarrow$) for ASR (gray).\ming{How about using a bar figure? I think the table is too small, and hard to read.}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
        \toprule
         \multirow{2}{*}{Datasets} & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{ABL} & \multicolumn{2}{c}{\method} \\
         \cline{2-7}  & ASR(\%) $\downarrow$ & ACC(\%) $\uparrow$  & ASR(\%) $\downarrow$ & ACC(\%) $\uparrow$  & ASR(\%) $\downarrow$ & ACC(\%) $\uparrow$ \\
        \midrule
         \textbf{AIDS} & \cellcolor{black!15} 100.00 & \textbf{96.20} & \cellcolor{black!15} 0.00 & 86.80 & \cellcolor{black!15} 0.00 & 94.20\\
         \textbf{PROTEINS} & \cellcolor{black!15} 100.00 & \textbf{66.42} & \cellcolor{black!15} 0.00 & 33.57 & \cellcolor{black!15} 0.00 & 65.69 \\
         \textbf{PROTEINS\_full} & \cellcolor{black!15} 100.00 & 71.30 & \cellcolor{black!15} 0.00 & 40.35 & \cellcolor{black!15} 0.00 &  \textbf{71.75} \\
         \textbf{ENZYMES} & \cellcolor{black!15} 100.00 & 35.83 & \cellcolor{black!15} 0.00 & 16.67 & \cellcolor{black!15} 0.00 & \textbf{38.83} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:maskcomp_data_iso}
\end{table}

\begin{table}[tbp]
    \centering
    \caption{Graph classification results on datasets selected by ground truth. Higher is better ($\uparrow$) for ACC (white). Lower is better ($\downarrow$) for ASR (gray).\ming{How about using a bar figure? I think the table is too small, and hard to read.}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cc|cc}
        \toprule
         \multirow{2}{*}{Datasets} & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{ABL} & \multicolumn{2}{c}{\method} \\
         \cline{2-7}  & ASR(\%) $\downarrow$ & ACC(\%) $\uparrow$  & ASR(\%) $\downarrow$ & ACC(\%) $\uparrow$  & ASR(\%) $\downarrow$ & ACC(\%) $\uparrow$ \\
        \midrule
         \textbf{AIDS} & \cellcolor{black!15} 100.00 & \textbf{96.20} & \cellcolor{black!15} 0.00 & 86.80 & \cellcolor{black!15} 0.00 & 96.00\\
         \textbf{PROTEINS} & \cellcolor{black!15} 100.00 & 66.42 & \cellcolor{black!15} 0.00 & 33.57 & \cellcolor{black!15} 0.00 & \textbf{78.53} \\
         \textbf{PROTEINS\_full} & \cellcolor{black!15} 100.00 & 71.30 & \cellcolor{black!15} 0.00 & 47.98 & \cellcolor{black!15} 0.00 &  \textbf{77.13} \\
         \textbf{ENZYMES} & \cellcolor{black!15} 100.00 & 35.83 & \cellcolor{black!15} 0.00 & 21.67 & \cellcolor{black!15} 0.00 & \textbf{45.00} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:maskcomp_gt}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

